The Surprising Positive Knowledge Transfer in Continual 3D Object Shape Reconstruction

Continual learning has been extensively studied for classification tasks with methods developed to primarily avoid catastrophic forgetting, a phenomenon where earlier learned concepts are forgotten at the expense of more recent samples. In this work, we present a set of continual 3D object shape reconstruction tasks, including complete 3D shape reconstruction from different input modalities, as well as visible surface (2.5D) reconstruction which, surprisingly demonstrate positive knowledge (backward and forward) transfer when training with solely standard SGD and without additional heuristics. We provide evidence that continuously updated representation learning of single-view 3D shape reconstruction improves the performance on learned and novel categories over time. We provide a novel analysis of knowledge transfer ability by looking at the output distribution shift across sequential learning tasks. Finally, we show that the robustness of these tasks leads to the potential of having a proxy representation learning task for continual classification. The codebase, dataset and pre-trained models released with this article can be found at https://github.com/rehg-lab/CLRec

==> figure/combine_task_arch.tex <==


% \begin{figure*}[t!]
% \vspace{-10pt}
% \centering
% \begin{minipage}{0.45\textwidth}
%     \includegraphics[width=\linewidth]{figure/shape_arch.pdf}
%     \vspace{-20pt}
%     \caption{An overview of a 3D shape reconstruction model. Given the shape feature encoded from the input and the 3D points, the MLP produces SDF values for each point. The zero-level set represents the surface of the object.}
%     \label{fig:arch}
% \end{minipage}
% \hspace{7pt}
% \begin{minipage}{0.5\textwidth}
% \centering
% \captionsetup{type=table} %% tell latex to change to table
% % \vspace{-10pt}
%     \caption{Summary of the reconstruction tasks we evaluate that demonstrate robustness to catastrophic forgetting. There are 5 types of tasks based on the input to output representation mapping.}
%     \vspace{-17pt}
% \input{tables/task_dataset}


%     \label{table:task}
% \end{minipage}
% \vspace{-20pt}
% \end{figure*}

\begin{figure*}[t!]
\vspace{-10pt}
\centering
\begin{minipage}{0.45\textwidth}
    \includegraphics[width=\linewidth]{figure/cl.pdf}
    \vspace{-20pt}
    \caption{An overview of a 3D shape reconstruction model. Given the shape feature encoded from the input and the 3D points, the MLP produces SDF values for each point. The zero-level set represents the surface of the object.}
    \label{fig:arch}
\end{minipage}
\hspace{7pt}
\begin{minipage}{0.5\textwidth}
\centering
\captionsetup{type=table} %% tell latex to change to table
% \vspace{-10pt}
    \caption{Summary of the reconstruction tasks we evaluate that demonstrate robustness to catastrophic forgetting. There are 5 types of tasks based on the input to output representation mapping.}
    \vspace{-17pt}
\input{tables/task_dataset}


    \label{table:task}
\end{minipage}
\vspace{-20pt}
\end{figure*}



% \begin{figure*}
% \begin{minipage}{0.5\linewidth}
% \centering
% \includegraphics[width=\linewidth]{figure/dist_bwt.pdf}
% \vspace{-10pt}
% \caption{Data variability in terms of pose, lighting and background.}
% \label{fig:rendering_effects}

% \end{minipage}
% \hspace{5pt}

% \begin{minipage}[t!]{.33\linewidth}

% \begin{table}[H]
% \scalebox{0.5}{
% \renewcommand{\arraystretch}{1.15}
% \centering


% \begin{tabular}{c|c|c|c}
%  Task  & Mean Dist. $\downarrow$ & BWT $\uparrow$ & FWT $\uparrow$ \\
% \hline
% Sil Pred. & 0.075 & -0.003 & 0.836\\
% VC 3D Shape Rec. & 0.077 & -0.123 &    0.105   \\    
% Depth Pred. & 0.084 & -0.136 & 0.094\\
% OC 3D Shape Rec. & 0.116 & -0.220 & 0.090\\
% Classification & 1 & -1 & -0.077\\
% \hline
% \end{tabular}
% }
    
%     \caption{The relationship between the mean output distribution distance across learning exposures and BWT and FWT for different CL tasks. Lower is better for distribution distance while higher is better for BWT and FWT. Lower distance leads to better knowledge transfer (higher BWT and FWT).}
%     \label{table:dist}

% % \begin{minipage}{0.55\linewidth}
% % \centering
% % \begin{table}[H]
% %     \input{tables/dist}
% %     % \vspace{-10pt}
% %     \caption{The relationship between the mean output distribution distance across learning exposures and BWT and FWT for different CL tasks. Lower is better for distribution distance while higher is better for BWT and FWT. Lower distance leads to better knowledge transfer (higher BWT and FWT).}
% %     \label{table:dist}
% % \vspace{-20pt}
% % \end{table}
% % \end{minipage}8
% \end{table}
% \end{minipage}
% \vspace{-5pt}
% \end{figure*}

==> tables/dist.tex <==
% \begin{center}
% \resizebox{\linewidth}{!}{

% \begingroup

% \setlength{\tabcolsep}{4pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.2} % Default value: 1


% \begin{tabular}{c|c|c|c}
%  Task  & Mean Dist. $\downarrow$ & BWT $\uparrow$ & FWT $\uparrow$ \\
% \hline
% Sil Pred. & 0.075 & -0.003 & 0.836\\
% VC 3D Shape Rec. & 0.077 & -0.123 &    0.105   \\    
% Depth Pred. & 0.084 & -0.136 & 0.094\\
% OC 3D Shape Rec. & 0.116 & -0.220 & 0.090\\
% Classification & 1 & -1 & -0.077\\
% \hline
% \end{tabular}
% \endgroup
% }

% \end{center}


\begin{center}
\resizebox{0.75\linewidth}{!}{

\begingroup

\setlength{\tabcolsep}{4pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1


\begin{tabular}{c|c|c|c}
 Task  & Normalized Mean Dist. $\downarrow$ & BWT $\uparrow$ & FWT $\uparrow$\\
\hline
Sil Pred. & 0.075 & -0.003 & 0.836 \\
VC 3D Shape Rec. & \textbf{0.076} & -0.123 &    0.105  \\    
Depth Pred. & 0.084 & -0.136 & 0.094 \\
OC 3D Shape Rec. & \textbf{0.105} & -0.220 & 0.090\\
\hline
\end{tabular}
\endgroup
}

\end{center}

